Key Focus Areas and Enabling Technologies for 6G

We provide a taxonomy of a dozen enabling network architectures, protocols, and technologies that will define the evolution from 5G to 6G. These technologies span the network protocol stack, different target deployment environments, and various perceived levels of technical maturity. We outline four areas of societal focus that will be impacted by these technologies, and overview several research directions that hold the potential to address the problems in these important focus areas.

==> sections-R4/ack.tex <==
\section{Acknowledgements}
This material is based in part upon work supported by the National
Science Foundation under grants.

